RIFT: Token Influence Follows the Path of Least Resistance

Which context tokens drive a language model's answer? Graph-based tools such as attention rollout and attention flow answer this from a single forward pass, yet their faithfulness in decoder-only models is rarely tested against interventions. We view the layers of a decoder as a causal network whose conductances are attention weights, and read a token's influence on the answer from the resistance between them. We propose RIFT (Resistance-based Information Flow in Transformers), which scores a token by the series resistance of its path of least resistance to the answer, found exactly by a classic shortest-path dynamic program. On synthetic in-context retrieval tasks and extractive question answering over Wikipedia paragraphs, RIFT predicts the effect of replacing a token with a Spearman correlation of 0.52-0.68; predicting a single replacement, it reaches 77-96% of the agreement between two different random replacements. It needs no gradients and no extra forward passes, scoring every token of a prompt in 0.9-3.4 ms on one CPU thread, whereas the replacement experiment needs a forward pass per token. On 576 held-out prompts from four models of two families (Qwen3 and Llama 3.2), it outperforms token distance, attention rollout and attention flow in every pre-specified comparison, by 0.23 to 0.88 in mean Spearman correlation, and it is the best or tied-best of all attention-based scores we test. Aggregates that add up all routes (attention flow, effective resistance and rollout) instead mostly encode token position: as a simple proposition shows, early tokens have many more parallel routes to the answer.

==> numbers.tex <==
\makeatletter
\newcommand{\val}[1]{\ifcsname rift@#1\endcsname\csname rift@#1\endcsname\else\textcolor{red}{\textbf{??#1??}}\fi}
\expandafter\def\csname rift@A-acc\endcsname{95}
\expandafter\def\csname rift@A-ceil\endcsname{0.61}
\expandafter\def\csname rift@A-plr\endcsname{0.53}
\expandafter\def\csname rift@A-ddist\endcsname{+0.41}
\expandafter\def\csname rift@A-ddist-lo\endcsname{+0.32}
\expandafter\def\csname rift@A-ddist-hi\endcsname{+0.49}
\expandafter\def\csname rift@A-droll\endcsname{+0.47}
\expandafter\def\csname rift@A-droll-lo\endcsname{+0.39}
\expandafter\def\csname rift@A-droll-hi\endcsname{+0.55}
\expandafter\def\csname rift@A-dflow\endcsname{+0.64}
\expandafter\def\csname rift@A-dflow-lo\endcsname{+0.55}
\expandafter\def\csname rift@A-dflow-hi\endcsname{+0.74}
\expandafter\def\csname rift@A-plrjac\endcsname{0.51}
\expandafter\def\csname rift@B-acc\endcsname{92}
\expandafter\def\csname rift@B-ceil\endcsname{0.71}
\expandafter\def\csname rift@B-plr\endcsname{0.63}
\expandafter\def\csname rift@B-ddist\endcsname{+0.63}
\expandafter\def\csname rift@B-ddist-lo\endcsname{+0.53}
\expandafter\def\csname rift@B-ddist-hi\endcsname{+0.72}
\expandafter\def\csname rift@B-droll\endcsname{+0.34}
\expandafter\def\csname rift@B-droll-lo\endcsname{+0.26}
\expandafter\def\csname rift@B-droll-hi\endcsname{+0.41}
\expandafter\def\csname rift@B-dflow\endcsname{+0.63}
\expandafter\def\csname rift@B-dflow-lo\endcsname{+0.55}
\expandafter\def\csname rift@B-dflow-hi\endcsname{+0.72}
\expandafter\def\csname rift@B-plrjac\endcsname{0.60}
\expandafter\def\csname rift@C-acc\endcsname{97}
\expandafter\def\csname rift@C-ceil\endcsname{0.67}
\expandafter\def\csname rift@C-plr\endcsname{0.53}
\expandafter\def\csname rift@C-ddist\endcsname{+0.42}
\expandafter\def\csname rift@C-ddist-lo\endcsname{+0.33}
\expandafter\def\csname rift@C-ddist-hi\endcsname{+0.50}
\expandafter\def\csname rift@C-droll\endcsname{+0.50}
\expandafter\def\csname rift@C-droll-lo\endcsname{+0.43}
\expandafter\def\csname rift@C-droll-hi\endcsname{+0.57}
\expandafter\def\csname rift@C-dflow\endcsname{+0.65}
\expandafter\def\csname rift@C-dflow-lo\endcsname{+0.57}
\expandafter\def\csname rift@C-dflow-hi\endcsname{+0.72}
\expandafter\def\csname rift@D-acc\endcsname{86}
\expandafter\def\csname rift@D-ceil\endcsname{0.67}
\expandafter\def\csname rift@D-plr\endcsname{0.55}
\expandafter\def\csname rift@D-ddist\endcsname{+0.64}
\expandafter\def\csname rift@D-ddist-lo\endcsname{+0.52}
\expandafter\def\csname rift@D-ddist-hi\endcsname{+0.75}
\expandafter\def\csname rift@D-droll\endcsname{+0.40}
\expandafter\def\csname rift@D-droll-lo\endcsname{+0.31}
\expandafter\def\csname rift@D-droll-hi\endcsname{+0.48}
\expandafter\def\csname rift@D-dflow\endcsname{+0.47}
\expandafter\def\csname rift@D-dflow-lo\endcsname{+0.37}
\expandafter\def\csname rift@D-dflow-hi\endcsname{+0.57}
\expandafter\def\csname rift@E-acc\endcsname{97}
\expandafter\def\csname rift@E-ceil\endcsname{0.59}
\expandafter\def\csname rift@E-plr\endcsname{0.59}
\expandafter\def\csname rift@E-ddist\endcsname{+0.74}
\expandafter\def\csname rift@E-ddist-lo\endcsname{+0.62}
\expandafter\def\csname rift@E-ddist-hi\endcsname{+0.86}
\expandafter\def\csname rift@E-droll\endcsname{+0.32}
\expandafter\def\csname rift@E-droll-lo\endcsname{+0.23}
\expandafter\def\csname rift@E-droll-hi\endcsname{+0.41}
\expandafter\def\csname rift@E-dflow\endcsname{+0.44}
\expandafter\def\csname rift@E-dflow-lo\endcsname{+0.33}
\expandafter\def\csname rift@E-dflow-hi\endcsname{+0.55}
\expandafter\def\csname rift@F-acc\endcsname{95}
\expandafter\def\csname rift@F-ceil\endcsname{0.62}
\expandafter\def\csname rift@F-plr\endcsname{0.52}
\expandafter\def\csname rift@F-ddist\endcsname{+0.58}
\expandafter\def\csname rift@F-ddist-lo\endcsname{+0.47}
\expandafter\def\csname rift@F-ddist-hi\endcsname{+0.69}
\expandafter\def\csname rift@F-droll\endcsname{+0.23}
\expandafter\def\csname rift@F-droll-lo\endcsname{+0.16}
\expandafter\def\csname rift@F-droll-hi\endcsname{+0.30}
\expandafter\def\csname rift@F-dflow\endcsname{+0.55}
\expandafter\def\csname rift@F-dflow-lo\endcsname{+0.47}
\expandafter\def\csname rift@F-dflow-hi\endcsname{+0.63}
\expandafter\def\csname rift@G-acc\endcsname{97}
\expandafter\def\csname rift@G-ceil\endcsname{0.67}
\expandafter\def\csname rift@G-plr\endcsname{0.60}
\expandafter\def\csname rift@G-ddist\endcsname{+0.70}
\expandafter\def\csname rift@G-ddist-lo\endcsname{+0.58}
\expandafter\def\csname rift@G-ddist-hi\endcsname{+0.81}
\expandafter\def\csname rift@G-droll\endcsname{+0.28}
\expandafter\def\csname rift@G-droll-lo\endcsname{+0.22}
\expandafter\def\csname rift@G-droll-hi\endcsname{+0.35}
\expandafter\def\csname rift@G-dflow\endcsname{+0.59}
\expandafter\def\csname rift@G-dflow-lo\endcsname{+0.50}
\expandafter\def\csname rift@G-dflow-hi\endcsname{+0.68}
\expandafter\def\csname rift@H-acc\endcsname{100}
\expandafter\def\csname rift@H-ceil\endcsname{0.67}
\expandafter\def\csname rift@H-plr\endcsname{0.68}
\expandafter\def\csname rift@H-ddist\endcsname{+0.88}
\expandafter\def\csname rift@H-ddist-lo\endcsname{+0.75}
\expandafter\def\csname rift@H-ddist-hi\endcsname{+0.99}
\expandafter\def\csname rift@H-droll\endcsname{+0.40}
\expandafter\def\csname rift@H-droll-lo\endcsname{+0.30}
\expandafter\def\csname rift@H-droll-hi\endcsname{+0.51}
\expandafter\def\csname rift@H-dflow\endcsname{+0.49}
\expandafter\def\csname rift@H-dflow-lo\endcsname{+0.37}
\expandafter\def\csname rift@H-dflow-hi\endcsname{+0.62}
\expandafter\def\csname rift@H-plrval\endcsname{0.57}
\expandafter\def\csname rift@H-pos-roll\endcsname{\ensuremath{-}0.91}
\expandafter\def\csname rift@I-acc\endcsname{100}
\expandafter\def\csname rift@I-ceil\endcsname{0.63}
\expandafter\def\csname rift@I-plr\endcsname{0.67}
\expandafter\def\csname rift@I-ddist\endcsname{+0.77}
\expandafter\def\csname rift@I-ddist-lo\endcsname{+0.65}
\expandafter\def\csname rift@I-ddist-hi\endcsname{+0.90}
\expandafter\def\csname rift@I-droll\endcsname{+0.30}
\expandafter\def\csname rift@I-droll-lo\endcsname{+0.22}
\expandafter\def\csname rift@I-droll-hi\endcsname{+0.38}
\expandafter\def\csname rift@I-dflow\endcsname{+0.59}
\expandafter\def\csname rift@I-dflow-lo\endcsname{+0.49}
\expandafter\def\csname rift@I-dflow-hi\endcsname{+0.68}
\expandafter\def\csname rift@I-plrval\endcsname{0.65}
\expandafter\def\csname rift@I-pos-roll\endcsname{\ensuremath{-}0.76}
\expandafter\def\csname rift@Mb-n\endcsname{192}
\expandafter\def\csname rift@Mb-acc\endcsname{98}
\expandafter\def\csname rift@Mb-ceil\endcsname{0.63}
\expandafter\def\csname rift@Mb-plr\endcsname{0.59}
\expandafter\def\csname rift@Mb-dist\endcsname{0.13}
\expandafter\def\csname rift@Mb-ddist\endcsname{+0.46}
\expandafter\def\csname rift@Mb-ddist-lo\endcsname{+0.41}
\expandafter\def\csname rift@Mb-ddist-hi\endcsname{+0.51}
\expandafter\def\csname rift@Mb-roll\endcsname{0.02}
\expandafter\def\csname rift@Mb-droll\endcsname{+0.56}
\expandafter\def\csname rift@Mb-droll-lo\endcsname{+0.51}
\expandafter\def\csname rift@Mb-droll-hi\endcsname{+0.61}
\expandafter\def\csname rift@Mb-flow\endcsname{\ensuremath{-}0.13}
\expandafter\def\csname rift@Mb-dflow\endcsname{+0.71}
\expandafter\def\csname rift@Mb-dflow-lo\endcsname{+0.65}
\expandafter\def\csname rift@Mb-dflow-hi\endcsname{+0.77}
\expandafter\def\csname rift@Mb-widest\endcsname{0.49}
\expandafter\def\csname rift@Mb-kirch\endcsname{\ensuremath{-}0.14}
\expandafter\def\csname rift@Mb-kirchjac\endcsname{\ensuremath{-}0.14}
\expandafter\def\csname rift@Mb-pos-plr\endcsname{0.19}
\expandafter\def\csname rift@Mb-pos-roll\endcsname{\ensuremath{-}0.73}
\expandafter\def\csname rift@Mb-pos-flow\endcsname{\ensuremath{-}1.00}
\expandafter\def\csname rift@Mb-pos-kirch\endcsname{\ensuremath{-}0.96}
\expandafter\def\csname rift@Mb-pos-widest\endcsname{0.07}
\expandafter\def\csname rift@Mi-acc\endcsname{94}
\expandafter\def\csname rift@Mi-ceil\endcsname{0.70}
\expandafter\def\csname rift@Mi-plr\endcsname{0.62}
\expandafter\def\csname rift@Mi-dist\endcsname{0.00}
\expandafter\def\csname rift@Mi-ddist\endcsname{+0.62}
\expandafter\def\csname rift@Mi-ddist-lo\endcsname{+0.56}
\expandafter\def\csname rift@Mi-ddist-hi\endcsname{+0.69}
\expandafter\def\csname rift@Mi-roll\endcsname{0.28}
\expandafter\def\csname rift@Mi-droll\endcsname{+0.34}
\expandafter\def\csname rift@Mi-droll-lo\endcsname{+0.30}
\expandafter\def\csname rift@Mi-droll-hi\endcsname{+0.38}
\expandafter\def\csname rift@Mi-flow\endcsname{0.00}
\expandafter\def\csname rift@Mi-dflow\endcsname{+0.62}
\expandafter\def\csname rift@Mi-dflow-lo\endcsname{+0.57}
\expandafter\def\csname rift@Mi-dflow-hi\endcsname{+0.67}
\expandafter\def\csname rift@Mi-widest\endcsname{0.61}
\expandafter\def\csname rift@Mi-kirch\endcsname{\ensuremath{-}0.01}
\expandafter\def\csname rift@Mi-kirchjac\endcsname{\ensuremath{-}0.02}
\expandafter\def\csname rift@Mi-pos-plr\endcsname{0.09}
\expandafter\def\csname rift@Mi-pos-roll\endcsname{\ensuremath{-}0.60}
\expandafter\def\csname rift@Mi-pos-flow\endcsname{\ensuremath{-}1.00}
\expandafter\def\csname rift@Mi-pos-kirch\endcsname{\ensuremath{-}0.91}
\expandafter\def\csname rift@Mi-pos-widest\endcsname{0.03}
\expandafter\def\csname rift@n-conf-word\endcsname{nine}
\expandafter\def\csname rift@n-comp\endcsname{27}
\expandafter\def\csname rift@L-pos-flow-min\endcsname{\ensuremath{-}0.67}
\expandafter\def\csname rift@L-pos-flow-max\endcsname{\ensuremath{-}0.55}
\expandafter\def\csname rift@C2-gpuh\endcsname{0.6}
\expandafter\def\csname rift@C3-gpuh\endcsname{0.5}
\expandafter\def\csname rift@C1-plr-min\endcsname{0.52}
\expandafter\def\csname rift@C1-plr-max\endcsname{0.68}
\expandafter\def\csname rift@C1-gapu-min\endcsname{0.23}
\expandafter\def\csname rift@C1-gapu-max\endcsname{0.88}
\expandafter\def\csname rift@C1-lowest-ci\endcsname{+0.16}
\expandafter\def\csname rift@C1-bestgapu-min\endcsname{0.23}
\expandafter\def\csname rift@C1-bestgapu-max\endcsname{0.42}
\expandafter\def\csname rift@C1-auc-plr-min\endcsname{0.95}
\expandafter\def\csname rift@C1-auc-plr-max\endcsname{0.99}
\expandafter\def\csname rift@C1-auc-roll-min\endcsname{0.58}
\expandafter\def\csname rift@C1-auc-roll-max\endcsname{0.73}
\expandafter\def\csname rift@C1-auc-flow-min\endcsname{0.43}
\expandafter\def\csname rift@C1-auc-flow-max\endcsname{0.61}
\expandafter\def\csname rift@C1-distlab-min\endcsname{\ensuremath{-}0.19}
\expandafter\def\csname rift@C1-distlab-max\endcsname{0.12}
\expandafter\def\csname rift@C1-auc-dist-min\endcsname{0.39}
\expandafter\def\csname rift@C1-auc-dist-max\endcsname{0.57}
\expandafter\def\csname rift@C1-pos-roll-min\endcsname{\ensuremath{-}0.91}
\expandafter\def\csname rift@C1-pos-roll-max\endcsname{\ensuremath{-}0.54}
\expandafter\def\csname rift@C1-pos-kirch-min\endcsname{\ensuremath{-}0.96}
\expandafter\def\csname rift@C1-pos-kirch-max\endcsname{\ensuremath{-}0.89}
\expandafter\def\csname rift@C1-gxi-min\endcsname{0.18}
\expandafter\def\csname rift@C1-gxi-max\endcsname{0.33}
\expandafter\def\csname rift@C1-widest-min\endcsname{0.48}
\expandafter\def\csname rift@C1-widest-max\endcsname{0.63}
\expandafter\def\csname rift@C1-kirch-min\endcsname{\ensuremath{-}0.14}
\expandafter\def\csname rift@C1-kirch-max\endcsname{0.14}
\expandafter\def\csname rift@C1-total-prompts\endcsname{576}
\expandafter\def\csname rift@S-total-prompts\endcsname{448}
\expandafter\def\csname rift@C1-gpuh\endcsname{2.7}
\expandafter\def\csname rift@M1-gpuh\endcsname{4.9}
\expandafter\def\csname rift@Mb-pos-rift\endcsname{\ensuremath{-}0.99}
\expandafter\def\csname rift@Mb-null-rift\endcsname{0.99}
\expandafter\def\csname rift@Mb-null-lab\endcsname{\ensuremath{-}0.13}
\expandafter\def\csname rift@Mi-pos-rift\endcsname{\ensuremath{-}0.98}
\expandafter\def\csname rift@Mi-null-rift\endcsname{0.98}
\expandafter\def\csname rift@Mi-null-lab\endcsname{0.00}
\expandafter\def\csname rift@toy-jac-pos-kirch\endcsname{\ensuremath{-}0.16}
\expandafter\def\csname rift@toy-att-pos-kirch\endcsname{\ensuremath{-}0.89}
\expandafter\def\csname rift@d3-kirch-k2\endcsname{\ensuremath{-}0.50}
\expandafter\def\csname rift@d3-kirch-k4\endcsname{\ensuremath{-}0.79}
\expandafter\def\csname rift@d3-roll-k2\endcsname{0.59}
\expandafter\def\csname rift@d3-roll-k28\endcsname{\ensuremath{-}0.66}
\expandafter\def\csname rift@d3-plr-k28\endcsname{0.14}
\expandafter\def\csname rift@C1-sgn-plr-min\endcsname{0.29}
\expandafter\def\csname rift@C1-sgn-plr-max\endcsname{0.47}
\expandafter\def\csname rift@C1-sgn-best-max\endcsname{0.20}
\expandafter\def\csname rift@C1-plrval-min\endcsname{0.51}
\expandafter\def\csname rift@C1-plrval-max\endcsname{0.62}
\expandafter\def\csname rift@M1-null-pos\endcsname{\ensuremath{-}1.00}
\expandafter\def\csname rift@Mi-null-pos\endcsname{\ensuremath{-}1.00}
\expandafter\def\csname rift@C1-tools-max\endcsname{0.37}
\expandafter\def\csname rift@task-first-n\endcsname{131}
\expandafter\def\csname rift@task-first-plr\endcsname{0.56}
\expandafter\def\csname rift@task-first-dist\endcsname{0.04}
\expandafter\def\csname rift@task-first-roll\endcsname{0.21}
\expandafter\def\csname rift@task-first-flow\endcsname{\ensuremath{-}0.04}
\expandafter\def\csname rift@task-first-ceil\endcsname{0.65}
\expandafter\def\csname rift@task-single-n\endcsname{283}
\expandafter\def\csname rift@task-single-plr\endcsname{0.55}
\expandafter\def\csname rift@task-single-dist\endcsname{\ensuremath{-}0.11}
\expandafter\def\csname rift@task-single-roll\endcsname{0.23}
\expandafter\def\csname rift@task-single-flow\endcsname{0.08}
\expandafter\def\csname rift@task-single-ceil\endcsname{0.62}
\expandafter\def\csname rift@task-twohop-n\endcsname{34}
\expandafter\def\csname rift@task-twohop-plr\endcsname{0.68}
\expandafter\def\csname rift@task-twohop-dist\endcsname{0.50}
\expandafter\def\csname rift@task-twohop-roll\endcsname{\ensuremath{-}0.03}
\expandafter\def\csname rift@task-twohop-flow\endcsname{\ensuremath{-}0.50}
\expandafter\def\csname rift@task-twohop-ceil\endcsname{0.84}
\expandafter\def\csname rift@task-squad-n\endcsname{128}
\expandafter\def\csname rift@task-squad-plr\endcsname{0.68}
\expandafter\def\csname rift@task-squad-dist\endcsname{\ensuremath{-}0.15}
\expandafter\def\csname rift@task-squad-roll\endcsname{0.32}
\expandafter\def\csname rift@task-squad-flow\endcsname{0.14}
\expandafter\def\csname rift@task-squad-ceil\endcsname{0.65}
\expandafter\def\csname rift@C1-len-min\endcsname{129}
\expandafter\def\csname rift@C1-len-max\endcsname{298}
\expandafter\def\csname rift@route-single-min\endcsname{94}
\expandafter\def\csname rift@route-single-max\endcsname{100}
\expandafter\def\csname rift@route-n\endcsname{576}
\expandafter\def\csname rift@route-layer-17\endcsname{20}
\expandafter\def\csname rift@route-layer-4b\endcsname{25}
\expandafter\def\csname rift@route-layer-llama\endcsname{16}
\expandafter\def\csname rift@route-layer-llama-hi\endcsname{19}
\expandafter\def\csname rift@route-q-n\endcsname{320}
\expandafter\def\csname rift@route-q-mode-pct\endcsname{87}
\expandafter\def\csname rift@route-q-near-pct\endcsname{99}
\expandafter\def\csname rift@route-llama-mode-pct\endcsname{51}
\expandafter\def\csname rift@route-layer-H\endcsname{20.5}
\expandafter\def\csname rift@route-layer-I\endcsname{19}
\expandafter\def\csname rift@exs-rho\endcsname{0.70}
\expandafter\def\csname rift@exs-median\endcsname{0.70}
\expandafter\def\csname rift@exs-tokens\endcsname{207}
\expandafter\def\csname rift@exs-question\endcsname{What type of animal did onlookers claim was piloting the boat?}
\expandafter\def\csname rift@exs-answer\endcsname{monkey}
\expandafter\def\csname rift@A-riftsingle\endcsname{0.49}
\expandafter\def\csname rift@A-dmax\endcsname{+0.05}
\expandafter\def\csname rift@A-dmax-lo\endcsname{+0.01}
\expandafter\def\csname rift@A-dmax-hi\endcsname{+0.10}
\expandafter\def\csname rift@A-dwid\endcsname{+0.05}
\expandafter\def\csname rift@A-dwid-lo\endcsname{+0.02}
\expandafter\def\csname rift@A-dwid-hi\endcsname{+0.08}
\expandafter\def\csname rift@A-dlog\endcsname{+0.03}
\expandafter\def\csname rift@A-dlog-lo\endcsname{\ensuremath{-}0.01}
\expandafter\def\csname rift@A-dlog-hi\endcsname{+0.06}
\expandafter\def\csname rift@A-comp\endcsname{single 32, first 32}
\expandafter\def\csname rift@B-riftsingle\endcsname{0.60}
\expandafter\def\csname rift@B-dmax\endcsname{+0.20}
\expandafter\def\csname rift@B-dmax-lo\endcsname{+0.15}
\expandafter\def\csname rift@B-dmax-hi\endcsname{+0.24}
\expandafter\def\csname rift@B-dwid\endcsname{+0.00}
\expandafter\def\csname rift@B-dwid-lo\endcsname{\ensuremath{-}0.03}
\expandafter\def\csname rift@B-dwid-hi\endcsname{+0.03}
\expandafter\def\csname rift@B-dlog\endcsname{+0.10}
\expandafter\def\csname rift@B-dlog-lo\endcsname{+0.08}
\expandafter\def\csname rift@B-dlog-hi\endcsname{+0.13}
\expandafter\def\csname rift@B-comp\endcsname{single 43, two-hop 21}
\expandafter\def\csname rift@C-riftsingle\endcsname{0.51}
\expandafter\def\csname rift@C-dmax\endcsname{+0.15}
\expandafter\def\csname rift@C-dmax-lo\endcsname{+0.11}
\expandafter\def\csname rift@C-dmax-hi\endcsname{+0.20}
\expandafter\def\csname rift@C-dwid\endcsname{\ensuremath{-}0.01}
\expandafter\def\csname rift@C-dwid-lo\endcsname{\ensuremath{-}0.03}
\expandafter\def\csname rift@C-dwid-hi\endcsname{+0.02}
\expandafter\def\csname rift@C-dlog\endcsname{+0.09}
\expandafter\def\csname rift@C-dlog-lo\endcsname{+0.06}
\expandafter\def\csname rift@C-dlog-hi\endcsname{+0.12}
\expandafter\def\csname rift@C-comp\endcsname{single 26, two-hop 13, first 25}
\expandafter\def\csname rift@D-riftsingle\endcsname{0.53}
\expandafter\def\csname rift@D-dmax\endcsname{+0.03}
\expandafter\def\csname rift@D-dmax-lo\endcsname{\ensuremath{-}0.01}
\expandafter\def\csname rift@D-dmax-hi\endcsname{+0.06}
\expandafter\def\csname rift@D-dwid\endcsname{+0.05}
\expandafter\def\csname rift@D-dwid-lo\endcsname{+0.01}
\expandafter\def\csname rift@D-dwid-hi\endcsname{+0.08}
\expandafter\def\csname rift@D-dlog\endcsname{+0.01}
\expandafter\def\csname rift@D-dlog-lo\endcsname{\ensuremath{-}0.02}
\expandafter\def\csname rift@D-dlog-hi\endcsname{+0.04}
\expandafter\def\csname rift@D-comp\endcsname{single 32, first 32}
\expandafter\def\csname rift@E-riftsingle\endcsname{0.54}
\expandafter\def\csname rift@E-dmax\endcsname{+0.18}
\expandafter\def\csname rift@E-dmax-lo\endcsname{+0.14}
\expandafter\def\csname rift@E-dmax-hi\endcsname{+0.23}
\expandafter\def\csname rift@E-dwid\endcsname{\ensuremath{-}0.01}
\expandafter\def\csname rift@E-dwid-lo\endcsname{\ensuremath{-}0.04}
\expandafter\def\csname rift@E-dwid-hi\endcsname{+0.03}
\expandafter\def\csname rift@E-dlog\endcsname{+0.09}
\expandafter\def\csname rift@E-dlog-lo\endcsname{+0.05}
\expandafter\def\csname rift@E-dlog-hi\endcsname{+0.12}
\expandafter\def\csname rift@E-comp\endcsname{single 64}
\expandafter\def\csname rift@F-riftsingle\endcsname{0.48}
\expandafter\def\csname rift@F-dmax\endcsname{+0.05}
\expandafter\def\csname rift@F-dmax-lo\endcsname{+0.01}
\expandafter\def\csname rift@F-dmax-hi\endcsname{+0.09}
\expandafter\def\csname rift@F-dwid\endcsname{+0.04}
\expandafter\def\csname rift@F-dwid-lo\endcsname{\ensuremath{-}0.01}
\expandafter\def\csname rift@F-dwid-hi\endcsname{+0.08}
\expandafter\def\csname rift@F-dlog\endcsname{+0.04}
\expandafter\def\csname rift@F-dlog-lo\endcsname{+0.01}
\expandafter\def\csname rift@F-dlog-hi\endcsname{+0.08}
\expandafter\def\csname rift@F-comp\endcsname{single 43, first 21}
\expandafter\def\csname rift@G-riftsingle\endcsname{0.55}
\expandafter\def\csname rift@G-dmax\endcsname{+0.11}
\expandafter\def\csname rift@G-dmax-lo\endcsname{+0.08}
\expandafter\def\csname rift@G-dmax-hi\endcsname{+0.15}
\expandafter\def\csname rift@G-dwid\endcsname{+0.04}
\expandafter\def\csname rift@G-dwid-lo\endcsname{+0.00}
\expandafter\def\csname rift@G-dwid-hi\endcsname{+0.08}
\expandafter\def\csname rift@G-dlog\endcsname{+0.10}
\expandafter\def\csname rift@G-dlog-lo\endcsname{+0.06}
\expandafter\def\csname rift@G-dlog-hi\endcsname{+0.14}
\expandafter\def\csname rift@G-comp\endcsname{single 43, first 21}
\expandafter\def\csname rift@H-rel12\endcsname{0.67}
\expandafter\def\csname rift@H-riftsingle\endcsname{0.63}
\expandafter\def\csname rift@H-lfl\endcsname{93}
\expandafter\def\csname rift@H-oracle\endcsname{0.61}
\expandafter\def\csname rift@H-riftnonrel\endcsname{0.44}
\expandafter\def\csname rift@H-relnonrel\endcsname{0.43}
\expandafter\def\csname rift@H-dmax\endcsname{+0.11}
\expandafter\def\csname rift@H-dmax-lo\endcsname{+0.08}
\expandafter\def\csname rift@H-dmax-hi\endcsname{+0.15}
\expandafter\def\csname rift@H-dwid\endcsname{+0.06}
\expandafter\def\csname rift@H-dwid-lo\endcsname{+0.03}
\expandafter\def\csname rift@H-dwid-hi\endcsname{+0.10}
\expandafter\def\csname rift@H-dlog\endcsname{+0.04}
\expandafter\def\csname rift@H-dlog-lo\endcsname{+0.01}
\expandafter\def\csname rift@H-dlog-hi\endcsname{+0.08}
\expandafter\def\csname rift@H-comp\endcsname{SQuAD 64}
\expandafter\def\csname rift@I-rel12\endcsname{0.63}
\expandafter\def\csname rift@I-riftsingle\endcsname{0.61}
\expandafter\def\csname rift@I-lfl\endcsname{96}
\expandafter\def\csname rift@I-oracle\endcsname{0.60}
\expandafter\def\csname rift@I-riftnonrel\endcsname{0.42}
\expandafter\def\csname rift@I-relnonrel\endcsname{0.44}
\expandafter\def\csname rift@I-dmax\endcsname{+0.07}
\expandafter\def\csname rift@I-dmax-lo\endcsname{+0.02}
\expandafter\def\csname rift@I-dmax-hi\endcsname{+0.12}
\expandafter\def\csname rift@I-dwid\endcsname{+0.05}
\expandafter\def\csname rift@I-dwid-lo\endcsname{+0.01}
\expandafter\def\csname rift@I-dwid-hi\endcsname{+0.09}
\expandafter\def\csname rift@I-dlog\endcsname{+0.07}
\expandafter\def\csname rift@I-dlog-lo\endcsname{+0.02}
\expandafter\def\csname rift@I-dlog-hi\endcsname{+0.12}
\expandafter\def\csname rift@I-comp\endcsname{SQuAD 64}
\expandafter\def\csname rift@C1-lfl-min\endcsname{77}
\expandafter\def\csname rift@C1-lfl-max\endcsname{96}
\expandafter\def\csname rift@C1-sbceil-min\endcsname{0.86}
\expandafter\def\csname rift@C1-sbceil-max\endcsname{0.91}
\expandafter\def\csname rift@C1-rel12-min\endcsname{0.59}
\expandafter\def\csname rift@C1-rel12-max\endcsname{0.71}
\expandafter\def\csname rift@C1-riftsingle-min\endcsname{0.48}
\expandafter\def\csname rift@C1-riftsingle-max\endcsname{0.63}
\expandafter\def\csname rift@C1-oracle-min\endcsname{0.65}
\expandafter\def\csname rift@C1-oracle-max\endcsname{0.70}
\expandafter\def\csname rift@C1-riftnonrel-min\endcsname{0.19}
\expandafter\def\csname rift@C1-riftnonrel-max\endcsname{0.33}
\expandafter\def\csname rift@C1-relnonrel-min\endcsname{0.29}
\expandafter\def\csname rift@C1-relnonrel-max\endcsname{0.43}
\expandafter\def\csname rift@C1-wid-siggap-min\endcsname{0.04}
\expandafter\def\csname rift@C1-wid-siggap-max\endcsname{0.06}
\expandafter\def\csname rift@C1-wid-tie-of\endcsname{4 of 9}
\expandafter\def\csname rift@C1-max-sig-of\endcsname{8 of 9}
\expandafter\def\csname rift@C1-log-sig-of\endcsname{7 of 9}
\expandafter\def\csname rift@C1-mean-sig-of\endcsname{8 of 9}
\expandafter\def\csname rift@C1-jac-wins-of\endcsname{6 of 7}
\expandafter\def\csname rift@C1-mg-wins-of\endcsname{5 of 7}
\expandafter\def\csname rift@C1-sgn-wins-of\endcsname{all nine}
\expandafter\def\csname rift@H-top-plr\endcsname{55}
\expandafter\def\csname rift@H-cleanacc\endcsname{72}
\expandafter\def\csname rift@I-top-plr\endcsname{60}
\expandafter\def\csname rift@I-cleanacc\endcsname{43}
\expandafter\def\csname rift@N-top-tools-max\endcsname{13}
\expandafter\def\csname rift@N-pool\endcsname{592}
\expandafter\def\csname rift@all-len-max\endcsname{307}
\expandafter\def\csname rift@N-tools-max\endcsname{0.37}
\expandafter\def\csname rift@Q-flow-exact\endcsname{383}
\expandafter\def\csname rift@Q-flow-n\endcsname{384}
\expandafter\def\csname rift@cost-rift-ms\endcsname{1.3}
\expandafter\def\csname rift@cost-rift-min-ms\endcsname{0.9}
\expandafter\def\csname rift@cost-rift-max-ms\endcsname{3.4}
\expandafter\def\csname rift@cost-roll-ms\endcsname{0.1}
\expandafter\def\csname rift@cost-rep-s-H\endcsname{4.4}
\expandafter\def\csname rift@cost-rep-s-I\endcsname{11.4}
\expandafter\def\csname rift@cost-flow-s\endcsname{73}
\expandafter\def\csname rift@cost-res-s\endcsname{56}
\expandafter\def\csname rift@cost-acc-rift\endcsname{0.62}
\expandafter\def\csname rift@cost-acc-rep\endcsname{0.65}
\expandafter\def\csname rift@cost-acc-roll\endcsname{0.29}
\expandafter\def\csname rift@cost-acc-flow\endcsname{0.12}
\expandafter\def\csname rift@cost-acc-res\endcsname{0.11}
\expandafter\def\csname rift@cost-ratio\endcsname{94}
\expandafter\def\csname rift@speedup-rep-min\endcsname{4{,}100}
\expandafter\def\csname rift@speedup-rep-max\endcsname{8{,}300}
\expandafter\def\csname rift@cost-n\endcsname{128}
\makeatother

